Iterative Geometry-Aware Cross Guidance Network for Stereo Image Inpainting

Currently, single image inpainting has achieved promising results based on deep convolutional neural networks. However, inpainting on stereo images with missing regions has not been explored thoroughly, which is also a significant but different problem. One crucial requirement for stereo image inpainting is stereo consistency. To achieve it, we propose an Iterative Geometry-Aware Cross Guidance Network (IGGNet). The IGGNet contains two key ingredients, i.e., a Geometry-Aware Attention (GAA) module and an Iterative Cross Guidance (ICG) strategy. The GAA module relies on the epipolar geometry cues and learns the geometry-aware guidance from one view to another, which is beneficial to make the corresponding regions in two views consistent. However, learning guidance from co-existing missing regions is challenging. To address this issue, the ICG strategy is proposed, which can alternately narrow down the missing regions of the two views in an iterative manner. Experimental results demonstrate that our proposed network outperforms the latest stereo image inpainting model and state-of-the-art single image inpainting models.

==> approach.tex <==
\section{Proposed Method}
%\qke{change the section name  to the name of your network?}
We first present the overall network architecture.
Then, we describe our GAA module and ICG strategy with details, respectively.
Finally, the training target functions are introduced.

\begin{figure*}[tb]
\centering
\includegraphics[width=0.8\linewidth]{fig2/structure.png}
\caption{Our proposed IGGNet network contains two key parts, a Geometry-aware Attention (GAA) module and an Iterative Cross Guidance (ICG) strategy. The
%parallel branches: a full-resolution branch and an encoder-decoder branch. 
Geometry-aware Attention (GAA) module explores the geometry correlation of the stereo pair and performs attention-driven feature aggregation. The Iterative Cross Guidance (ICG) strategy exploits the guidance through a confidence-driven mask updating module to alternately shrink the missing regions of the two views.}
\label{fig:structure}

\end{figure*}


\subsection{Network Overview}
Given a rectified stereo image pair $(X_{left}, X_{right})$ annotated with binary masks $(M_{left}, M_{right})$, the goal of our network is to generate the output pair $(\hat{Y}_{left},\hat{Y}_{right})$.
The output pair should not only have visually plausible restored contents but also maintain the geometry consistency with the ground truth pair $(Y_{left},Y_{right})$.
To achieve this goal, we restore the two images in an iterative manner with the proposed \textbf{Iterative Cross Guidance (ICG)} strategy  using the deep network containing a \textbf{Geometry-Aware Attention (GAA)} module.

Specifically, 
for the first iteration, we take the left view $X_{left}$ as the target (the view to be inpainted) and the right view $X_{right}$ as the reference (guidance).
As shown in Figure~\ref{fig:structure} (a), the IGGNet includes two  parallel branches: an encoder-decoder branch and a full resolution branch.
We implement Gated convolution \cite{Yu_2019_ICCV} as the basic convolution operation in both branches.
For the encoder-decoder branch, both the target and reference images are fed into the encoding network, which generates the corresponding feature maps $\phi_{tar}$ and $\phi_{ref}$, respectively.
The two feature maps are processed by the  %\textbf{Geometry-Aware Attention (GAA)}
GAA module, which explores the geometry correspondence between them and incorporates most relevant context from $\phi_{ref}$ to guide the inpainting of $\phi_{tar}$ (More details are explained in Section~\ref{secGAA}).  
Then, the decoding network decodes the aggregated feature maps (output of the GAA module) to a restored target image. In addition,
the full resolution branch consists of four  consecutive full-resolution Gated convolution \cite{Yu_2019_ICCV} layers, which are beneficial to the maintenance of high-resolution representations \cite{Guo2019ProgressiveII}.
The outputs of two parallel branches are then fused through the element-wise addition operation. 

After the first iteration, we obtain the inpainted left image $X_{left}^{1}$ with narrowed missing regions, as shown in Figure~\ref{fig:structure} (a).
Next, we swap the roles of the two images, {\it i.e.,} the inpainted left image $X_{left}^{1}$ as the reference and the original right images $X_{right}$ as the target, and then feed them to the second iteration, which yields the inpainted right image $X_{right}^1$.  
In the following iterations, we continue to swap the roles of target and reference, {\it e.g.,} $X_{left}^1$ (target) and $X_{right}^1$ (reference) as input for the third iteration, and repeat the cross guidance process over $T$ iterations in total to obtain the final restored images $\hat{Y}_{left}$ and $\hat{Y}_{right}$. 


%To address the disturbance from the co-existing missing regions in the stereo pair, we propose the \textbf{Iterative Cross Guidance (ICC)} strategy.
%With the ICG strategy, the left and right images can crossly guide each other and alternately improve their results by progressively filling holes with a confidence-driven mask updating module.
%As shown in Figure~\ref{fig:structure}, the network narrows down the missing region in the target image $X_{left}$ by trusting only high-confidence pixels inside the hole, and get the restored left image $X_{left}^{1}$ for the first iteration.
%Then for the second iteration, we take $X_{left}^{1}$ as the reference and $X_{right}$ as the target, and the rest iterations are done so on.

\subsection{Geometry-Aware Attention Module}\label{secGAA}
In this section, we introduce the GAA module by taking the example of the left image as the target and the right as the reference. Since the missing content of the left image might occur in the right one, it is crucial to take advantage of the right image as the guidance to inpaint the left. To achieve this, we can warp the right image according to the disparity map~\cite{liang2018learning}, which indicates the displacement between the corresponding pixels of the two views, and then directly exploit the warped image as the guidance. However, the disparity information is often unavailable, which can be obtained by traditional SGM algorithms~\cite{hirschmuller2005accurate} or deep learning based approaches~\cite{liang2018learning}. Both of them require extra computational and time costs. 
Additionally, if there are  missing regions or noises in the disparity map, we also need to process the disparity map firstly. 
To deal with this issue, 
We capitalize on the epipolar geometry of the stereo images, {\it i.e.,} the corresponding pixel of the pixels in one view lies on the epipolar line of the other view.
%\qke{again explain a bit in case the reviewers from inpainting do not know this} 
Specifically, we  learn an attention map, which provides the identical information to the disparity map, upon the $4$D cost-volume \cite{Kendall_2017_ICCV,Chang_2018_CVPR,Zhang_2019_CVPR} created from the two images. 
As a result, our model is able to adaptively capture the useful information from the reference to guide the restoration of the target without the requirement of disparity information. 
%\qke{briefly talk about the benefit of this method, how it handles the cost and time consuming problem in getting disparity map)}
Next, we provide more details.

As shown in Figure~\ref{fig:structure} (b), the GAA module first builds a cost volume upon the encoded feature maps $\phi_{tar}\in \mathbb{R}^{H\times W \times C}$ and $\phi_{ref} \in \mathbb{R}^{H\times W \times C}$  by concatenating the target feature map with their corresponding reference feature maps across every disparity level, resulting in a 4D volume $V \in \mathbb{R}^{H\times W \times D \times 2C}$.
Here $D$ denotes the predefined maximum disparity value, which is set as $192$ in our experiments.
In order to aggregate the feature information 
along the disparity dimension as well as the channel dimension, 
we first apply consecutive 3D convolutional operations on the channel dimension followed by a Softmax operation on the disparity dimension to get a $4$D attentional map $A \in \mathbb{R}^{H\times W \times D \times C}$. 
We then perform an attention-driven feature aggregation to update the features of the target adaptively.
%\qke{how adaptive? and why use the following method}
Specifically, we apply element-wise product on $A$ and $V_{ref}\in\mathbb{R}^{H\times W \times D \times C}$, where $V_{ref}$ represents the corresponding part of the reference view in $V$,
%\qke{A is 4d, phi is 3d? how element wise product?}
and sum the elements  along the disparity dimension (the third dimension) to obtain the attended reference feature map $\phi_{ref\_atn} \in \mathbb{R}^{H\times W \times C}$:

\begin{equation}
\phi_{ref\_atn} = \sum_{d=0}^{D}A\times V_{ref},
\end{equation}

Finally, we concatenate $\phi_{tar}$ and $\phi_{ref\_atn}$ on the channel dimension as the output of GAA module.







\subsection{Iterative Cross Guidance}
The co-existing missing regions in the stereo image pair make the inpainting task extremely challenging. When the model uses the reference view as guidance to inpaint the target view, missing regions in the reference view inevitably causes inaccurate attention computation and feature aggregation.
Therefore, we propose an iterative cross guidance inpainting strategy. 
The whole inpainting procedure is composed of a number $T$ of inpainting iterations, in which the two views alternately serve as the target view and reference view, respectively.
Each view is inpainted by $T/2$ times ($T$ is supposed to be an even number).
In each iteration, we shrink the missing region in the target view with a confidence-driven mask updating module using the model with the proposed GAA module.



\noindent\textbf{Confidence-Driven Mask Updating} 
We observe that in the failure cases of existing approaches, despite the artifacts,
there often exist sub-regions with plausible predictions. 
By trusting the plausible part and treating the remaining part as a new mask, we can run the network again and again.
In this way, the mask becomes progressively smaller and the model can produce better results.
Inspired by this observation, we exploit a confidence-driven mask updating module to keep the inpainted region with higher confidence in the target image but ignore those with large prediction error.
To realize the mask confidence prediction, we utilize the Gated Convolution \cite{Yu_2019_ICCV} in both the full-resolution and the encoder-decoder branches instead of the standard 2D convolution.
Specifically, we modify the last Gated convolution layer of the two branches by setting a confidence threshold on the generated three-channel soft mask $m \in [0,1]^{H\times W \times 3}$, and obtain the updated one-channel binary mask $M\in \{0,1\}^{H\times W \times 1}$.


\begin{equation}
  M(i,j)=\left\{
  \begin{array}{@{}ll@{}}
    1, & \text{if}\ \max[m(i,j,:)]>0.5) \\  
    0, & \text{otherwise}
  \end{array}\right.
\end{equation} 

Algorithm 1 illustrates the overall procedure of the ICG strategy.


\begin{algorithm}[H]
\algsetup{linenosize=\small}
\caption{Iterative Cross Guidance}
\label{ALG1}
%\normalsize
\small
%\scriptsize
\begin{algorithmic}[1]
\REQUIRE number of iterations $T$, left input image $X_{left}$, right input image $X_{right}$, full resolution branch $\text{Branch\_f}$, encoder-decoder branch $\text{Branch\_ed}$ 
\ENSURE restored left image $\hat{Y}_{left}$, restored right image $\hat{Y}_{right}$ 
\STATE $X_{tar}^{0} = X_{left}, X_{ref}^{0} = X_{right}$
\FOR{$t$ in ${1,...,T}$}
\STATE $ R_{f}, m_{f} = \text{Branch\_f}(X_{tar}^{t-1})$
\STATE $ R_{ed}, m_{ed} = \text{Branch\_ed}(X_{tar}^{t-1}, X_{ref}^{t-1})$
\STATE $M_{f} = \text{Formula\_2}(m_{f})$
\STATE $M_{ed} = \text{Formula\_2}(m_{ed})$
\STATE $M_{t} = M_{f} \bigodot M_{ed}$
\STATE $R^{t} = \frac{1}{2}(M_{t} \bigodot (R_{f} + R_{ed}))$
\STATE $X_{tar}^{t} = X_{ref}^{t-1}$
\STATE $X_{ref}^{t} = R^{t}$
\IF{$t \%  2 == 1$}
\STATE $X_{left}^{(t+1)/2} = R^{t}$
\ELSE
\STATE $X_{right}^{t/2} = R^{t}$
\ENDIF
\ENDFOR
\STATE $\hat{Y}_{left} = X_{left}^{T/2}, \hat{Y}_{right} = X_{right}^{T/2}$

\end{algorithmic}
\end{algorithm}





\subsection{Loss Function}
The loss function used for training is:

\begin{equation}
\mathcal{L}_{total} = \mathcal{L}_{\text{rec}} + \lambda_{\text{adv}}\mathcal{L}_{\text{adv}},
\end{equation}
Here, $\mathcal{L}_{\text{rec}}$ and $\mathcal{L}_{\text{adv}}$ denote reconstruction loss and adversarial loss respectively.
The balancing weight $\lambda_{\text{adv}}$ is empirically set to 0.01. 

\begin{equation}
\mathcal{L}_{\text{rec}} = \sum_{t}^{T/2}\|(X_{left}^{t} - Y_{left}) + (X_{right}^{t} - Y_{right})\|_{1},
\end{equation}

\begin{equation}
\begin{split}
\mathcal{L}_{\text{adv}} & = \sum_{t}^{T/2} (\log(Dis(Y_{left})) + \log(1 - Dis(X_{left}^{t})) \\ & + \log(Dis(Y_{right})) + \log(1 - Dis(X_{right}^{t})) ),
\end{split}
\end{equation}


where $Dis$ denotes the discriminator of GAN \cite{goodfellow2014generative}. We also adopt spectral normalization \cite{Miyato2018SpectralNF} to stabilize the convergence of the discriminator.
Here the generator $G$ of the GAN is the IGGNet.
$G$ and $D$ are trained simultaneously by solving $\arg min_{G} max_{D} \mathcal{L}_{\text{adv}}$.

==> intro.tex <==
\section{Introduction}\label{secIntro}
Image inpainting aims to synthesize alternative contents in the missing regions of an image given a corresponding mask.
It has a wide range of applications such as photo recovery and object removal.
Recent years have witnessed promising results on inpainting individual images  with deep learning-based approaches.
Through automatically acquiring intrinsic hierarchical representations, these approaches~\cite{liu2018image,Yu_2019_ICCV,Li_2020_CVPR,Zeng_2021_ICCV} can perceive the image content and generate high-level semantic features to restore the missing contents. 
%Such approaches mostly outperform traditional image inpainting methods \cite{bertalmio2003simultaneous,barnes2009patchmatch}. 
Further attempts~\cite{kim2019deep,xu2019deep} have been made to tackle the inpainting problem over an image sequence, {\it a.k.a} video inpainting, through considering the temporal information. 




\begin{figure}[t!]
    \centering
    \setlength{\tabcolsep}{0.05em}
    {
\begin{tabular}{ccccc}
        
\rotatebox[origin=l]{90}{\small Left}&
\includegraphics[width=1.9cm]{fig1/input_l.png}&
\includegraphics[width=1.9cm]{fig1/output_l_GC.png}&
\includegraphics[width=1.9cm]{fig1/output_l_our.png}&
\includegraphics[width=1.9cm]{fig1/gt_l.png}\\

\addlinespace[-0.20em]

\rotatebox[origin=l]{90}{\small Right}&
\includegraphics[width=1.9cm]{fig1/input_r.png}&
\includegraphics[width=1.9cm]{fig1/output_r_GC.png}&
\includegraphics[width=1.9cm]{fig1/output_r_our.png}&
\includegraphics[width=1.9cm]{fig1/gt_r.png}\\

  & \small Input   & \small SICNet    & \small IGGNet   & \small  GT \\
  
\end{tabular}  

}
\caption{An example of visual comparison with state-of-the-art single image inpainting model SICNet~\cite{yu2018generative} on a stereo pair (which contains two images, i.e.,  left view and right view) from the  KITTI2015 dataset~\cite{mayer2016large}. GT is the ground truth image. As shown here, the input stereo pair can have different missing regions in each view. The proposed IGGNet is effective to incorporate geometry correlation and generate stereo consistent results.}
\label{example}
\end{figure}




%\qke{the motivation of stereo image inpating is not very strong, you  may also state the benefit of using stereo iamges. you may also describe this new task because maybe inpating reviewer are not familiar with stereo images}
Stereo images are becoming a type of prevalent media due to the use of head-mounted devices ({\it e.g.,} AR/VR glasses) and dual-lens smart phones. 
Inpainting on stereo images can realize many functionalities such as object removal, content editing, privacy protection, which will benefit a wide range of applications (autonomous driving, AR/VR softwares, {\it etc.}).
%Studies based on stereo images have sprouted, such as stereoscopic style transfer \cite{Gong_2018_ECCV, Chen_2018_CVPR} and super resolution \cite{Wang_2019_CVPR, Yan_2020_CVPR}. 
However, inpainting stereo images has not yet been explored thoroughly. 
%However, to the best of our knowledge, there are no deep learning techniques that  address the inpainting problem of stereo images.
%In this paper, we address the need for this booming 3D media by proposing the first deep stereo image inpainting model. 
A straightforward solution is to directly apply single image inpainting methods (developed for individual images) over the left view and the right view separately. 
However, this may lead to severe stereo inconsistency, because inpainting an individual image only considers the undamaged spatial statistics in that image, {\it i.e.,} only one view of the stereo images, but ignores the geometric relationship between the two views. 
Here, stereo inconsistency refers to that the inpainted stereo pair, {\it i.e.,} the left and the right output images, has different structures or textures in the same region. 
While Ma \etal~\shortcite{Ma2020LearningAV} recently propose the SICNet for stereo image inpainting, it is unable to effectively explore the stereo cues as shown in in Figure~\ref{example}.


Based on the above observations and analysis, we summarize two crucial and distinctive problems for stereo image inpainting:
(1) How to effectively take advantage of the epipolar geometry cues in the stereo images.
Here, epipolar geometry cues refer to that a region, which is missing in one view, might be undamaged in another view and can be found in the epipolar line.
This is essential for generating stereo consistent results.
(2) How to alleviate the impact of co-existing missing regions in the stereo images.
This refers to the fact that there might exist some regions which are missing in both two views.
When using one view as the reference view to guide the inpainting of the other view, {\it i.e.,} the target view, missing regions in the reference view inadvertently cause disturbance on the incorporation of geometry correlation. 
%Under such circumstances, the stereo correlations in a region which is missing in both views are difficult to build.






To address the two problems above, we propose a stereo inpainting network named the \textbf{Iterative Geometry-Aware Cross Guidance Network (IGGNet)}. 
This network explores and integrates the stereo geometry, and performs inpainting on the two images ({\it i.e.,} left view and right view) in an iterative manner. 
There are two key ingredients in the proposed network, {\it i.e.,}   \emph{Geometry-Aware Attention} (GAA) module and a \emph{Iterative Cross Guidance} (ICG) strategy.  The GAA module explicitly learns attention maps based on the epipolar geometry of stereo images to exploit the guidance from one view (reference) to another one (target).
%, and then aggregate the attention-driven features to update the features of the target view. 
The ICG strategy alternately narrows down the missing regions in the two views to alleviate the impact of co-existing missing regions and is beneficial to obtain better visual consistency in the inpainted results. 
More specifically, 
in a certain iteration, we take one view as the target view (the view to be inpainted) and the other one as the reference (guidance). Given the inpainted target view obtained after this iteration and the reference view, %we infer and gather a new missing region boundary of the inpainted target view with a confidence-driven mask updating module.
we swap the roles of them, {\it i.e.,} the reference and the target, as the input for  the next iteration, and so on for the following iterations. 
By processing the two views using the geometry-aware cross guidance in an iterative manner, our model is able to yield high-quality inpainting results with better geometry consistency from the stereo images with masks.  

%To exploit the guidance from one view (reference) to another one (target), we design the \emph{Geometry-Aware Attention} (GAA) module that can explicitly learn attention maps based on the epipolar geometry of stereo images. Then, attention-driven feature aggregation is performed to update the features of the target view. To alleviate the impact of co-existing missing regions and obtain better visual consistency in the inpainted results, we present an \emph{Iterative Cross Guidance} (ICG) strategy to alternately narrow down the missing regions in the two views.In a certain iteration, we take one view as the target view (the view to be inpainted) and the other view as the reference view (guidance).Specifically, we infer and gather the new missing region boundary of the inpainted target view with a confidence-driven mask updating module.Then we swap the target and reference views as the input for the next iteration, and so on for the following iterations. By processing the two views using the geometry-aware cross guidance in an iterative manner, our model is able to yield high-quality inpainting results with better geometry consistency from the stereo images with masks. 


In summary, our main contributions are:
\begin{itemize}

  \item We propose a novel end-to-end network for stereo image inpainting, which can take effective advantage of the geometry correspondence between the stereo views and crossly do the inpainting in an iterative manner.

 
  \item We introduce a \textit{Geometry-Aware Attention} (GAA) module that incorporates the correlation between the two views of a stereo pair based on the epipolar geometry. 
  The GAA module takes effective advantage of epipolar geometry cues and directly benefits generating stereo consistent results.
  
  \item We adopt an \textit{Iterative Cross Guidance} (ICG) strategy that  exploits the geometry-aware guidance to alternately shrink the missing regions of the two views. In this way, we can alleviate the disturbance from the co-existing missing regions in the stereo pair.

  
  \item Experiments on real data demonstrate that our proposed IGGNet outperforms conventional stereo inpainting methods and state-of-the-art models designed for  
    single image or video inpainting problems.
\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Introduction}\label{secIntro}
%Stereo images are standing on the trend of becoming a prevalent media due to the widespread of head-mounted devices (e.g., AR/VR glasses) and dual-lens smart phones. Interesting research works based on stereo images have sprouted out, such as stereoscopic style transfer \cite{Gong_2018_ECCV, Chen_2018_CVPR} and super resolution \cite{Wang_2019_CVPR, Yan_2020_CVPR}. Besides these studies, synthesizing stereoscopic contents is always intriguing.

%Image inpainting aims at synthesizing alternative contents in the missing regions of an image given a corresponding mask.
%It has a wide range of applications such as photo recovery and object removal.
%Recent years have witnessed promising development on single image inpainting with deep learning-based approaches. 
%By automatically acquiring intrinsic hierarchical representations, these methods \cite{pathak2016context,iizuka2017globally,Yang_2017_CVPR,liu2018image,yu2018generative,Xiong_2019_CVPR,zeng2019learning,Yu_2019_ICCV} can perceive the image content and generate high-level semantic features to restore the missing contents, which generally outperform the traditional image inpainting methods \cite{bertalmio2003simultaneous,barnes2009patchmatch}. 

%However, the possibility of applying deep learning-based inpainting to stereo images has not yet been sufficiently explored.
%For stereo image inpainting, one straight-forward solution is to directly apply single image inpainting methods to the left view and right view individually. 
%However, this will lead to severe view inconsistency which disturbs the original epipolar-geometry dependency incorporated in the stereo pair and thus brings users an uncomfortable visual experience. 
%Here view inconsistency refers to that the inpainted stereo pair has different restored structures or textures within the same missing regions from the input. 
%This is because single image inpainting only consider the undamaged spatial statistics in one view and ignores the epipolar-geometry dependency betweeen the two views. 
%Specifically, a region which is missing in one view can be undamaged in another view along the same epipolar plane, which provide strong cues for inpainting.
%An example is shown in Figure~\ref{}, where restored patterns of the same missing region in the two views are obviously inconsistent.
%Another possible solution is to use video inpainting methods, which consider the temporal consistency and utilize the adjacent frames as reference information. 
%However, different from videos which are recorded at the same viewpoint and different time points, stereo images are characteristic of different viewpoints at the same time. 
%In order to incorporate many reference frames, video inpainting methods usually have complicated procedures with multiple stages, which makes it inappropriate to directly apply video inpainting methods on stereo images.
%Moreover, different from stereo image style transfer or super resolution, the fact that the left view image and the right view image both have missing regions with different shapes and sizes will bring extra challenges for stereo image inpainting.
%Under such circumstances, the stereo correlations in an area where in both views are missing are extremely hard to build and the network will generate semantically ambiguous results.
%Therefore, it is essential to simultaneously consider how to effectively utilize the corresponding epipolar geometry cues and how to alleviate the impact of different missing regions in the two views for high-quality stereo image inpainting.

%In this paper, we aim to address the challenges above in a principled manner from the following three aspects: 
%(1) We propose an \textbf{Epipolar Geometry-guided Recurrent network (EGRnet)} for stereo image inpainting, which can not only fully explore and integrate the stereo correspondence, but also perform inpainting on the two view images in a progressive manner.
%(2) To better exploit the epipolar geometry between the two view images, we propose a \emph{Epipolar Geometry-guided Attention} (EGA) module.
%Given a stereo image pair with missing regions on both views, we first extract their feature maps using a shared encoding network.
%Then, the two feature maps are fed to EGA to exploit the epipolar geometry between them.
%Specifically, this module first constructs a 4D cost volume by concatenating the left feature map with the corresponding right feature map across different disparity levels.
%An attention map is generated by feeding the cost volume into a 3D CNN for computing feature similarities with all possible disparity values. 
%After that, attention-driven feature aggregation is performed to update the features of the left image. 
%Finally, the updated feature map is forwarded to the decoding network to generate the inpainting result.
%(3) To alleivate the impact of coexisting missing regions in the stereo image pair, we design a recurrent framework to alternately narrow down the missing regions in the two views.
%For a certain iteration, we take one view as the target view (the view to be inpainted), and the other view as the reference view.
%After inferring and gathering the new hole boundary for the target view, we then swap the target and reference as the input for the next iteration.

%In summary, our main contributions are:
%\begin{itemize}
%  \item We propose a novel end-to-end network for stereo image inpainting. The model can effectively integrate the epipolar geometry correspondence in a progressive manner.

%  \item We propose a \textit{Epipolar Geometry-guided Attention} (EGA) module, which exploits the correlation between the two views and strengthens the geometry constraints for estimating pixels. The EGA module not only significantly enhances network performance but also address limitations of single image or video inpainting methods.
  
%  \item We propose a recurrent framework, which utilizes a learning-based mask updating policy to alternately shrink the missing regions of the two views. In this way, we natually alleviate the disturbance from the coexisting missing regions in the stereo pair.

  
%  \item Experiments empirically demonstrate our proposed network’s superiority
%to the state-of-the-art single image or video inpainting methods.
%\end{itemize}









